Nearly Linear Row Sampling Algorithm for Quantile Regression

We give a row sampling algorithm for the quantile loss function with sample complexity nearly linear in the dimensionality of the data, improving upon the previous best algorithm whose sampling complexity has at least cubic dependence on the dimensionality. Based upon our row sampling algorithm, we give the fastest known algorithm for quantile regression and a graph sparsification algorithm for balanced directed graphs. Our main technical contribution is to show that Lewis weights sampling, which has been used in row sampling algorithms for $\ell_p$ norms, can also be applied in row sampling algorithms for a variety of loss functions. We complement our theoretical results by experiments to demonstrate the practicality of our approach.

==> alg.tex <==
%!TEX root = main.tex

\section{Algorithm for Approximating Leverage Scores and $\ell_1$ Lewis Weights} \label{sec:alg}
In this section, we sketch how to approximate leverage scores and $\ell_1$ Lewis weights of a matrix $A = [B ~ c] \in \mathbb{R}^{m \times (n + 1)}$, where $B\in \mathbb{R}^{m \times n}$ is the capacitated edge-vertex incidence matrix of a graph $G = (V, E)$ and $c \in \mathbb{R}^{m}$ is an arbitrary cost vector, in $\widetilde{O}(m)$ time.
Here, we assume $G$ is connected, since otherwise, we can run the algorithm on each connected component of $G$ separately. We also assume the cost vector $c$ is not in the column space of $B$, since otherwise, we can directly return the leverage scores or the $\ell_1$ Lewis weights of $B$. Furthermore, we can check whether $c$ is in the column space of $B$ or not, in $O(m)$ time, by regarding $c$ as a vector of current and checking whether $c$ admits Kirchhoff's Voltage Law (KVL). 

For the purpose of Theorem \ref{thm:quantile-sample}, it suffices to obtain $O(1)$-approximations to the  $\ell_1$ Lewis weights of $A$. 
Using \cite{cohen2015p}, it suffices to design an algorithm that returns $O(1)$-approximations to the leverage scores of $WA$, for positive diagonal matrices $W \in \mathbb{R}^{m \times m}$. Note that $WA = [WB ~ Wc]$ is of the same form as $A$ and $WB$ is the edge-vertex incidence matrix of a reweighted $G$, the rest of the section is thus devoted to devising algorithms for obtaining constant-factor approximations to leverage scores of $A$.

The leverage scores of a matrix $A$ are $a_i^T(A^TA)^\dagger a_i = \|A(A^TA)^\dagger a_i\|_2^2$, where $a_i$ is the $i$-th row of $A$, and therefore it suffices to calculate $GA(A^TA)^{\dagger}$, for a Johnson-Lindenstrauss matrix $G \in \mathbb{R}^{O(\log n) \times m}$~\cite{spielman2011graph, koutis2012improved}. 
We may first calculate $GA$ in $\widetilde{O}(m)$ time and now it suffices to calculate $g^T(A^T A)^{\dagger}$ for each row $g^T$ of $GA$.
Since there are only $O(\log n)$ rows in $GA$, in order to obtain an algorithm that runs in $\widetilde{O}(m)$, it would be sufficient to calculate $g^T(A^T A)^{\dagger}$ in $\widetilde{O}(m)$ time. 

Notice that
$$
A^TA = \left[ \begin{array}{cc} B^T B & B^T c \\ c^TB  &  c^Tc\end{array}\right],
$$
where $L = B^TB$ is the weighted Laplacian matrix of $G$ (recall that $B$ has been reweighted by a diagonal matrix $W$).
Since $G$ remains connected after reweighting, $\rank(L) = \rank(B^TB) = n - 1$ and the orthogonal complement of the column space of $L$ is the subspace spanned by $\mathbf{1}$.
Moreover, $B^Tc$ is in the column space of $L$ since $\mathbf{1}^T (B^T c) = 0$.
Similarly, $c^TB$ is in the row space of $L$.
Furthermore, since $c$ is not in the column space of $B$, we have $\rank(A^TA) = \rank(L) + 1 = n$.
To summarize, we have
\begin{itemize}
\item $LL^{\dagger} B^T c = B^T c$;
\item $c^T B L^{\dagger} L = c^TB$;
\item $c^T B L^{\dagger} B^T c \neq c^T c$.
\end{itemize}
At this point we use (2.1) in \cite{miao1991general}, obtaining
$$
(A^TA)^{\dagger} = \left[ \begin{array}{cc} L^{\dagger} + L^{\dagger} B^T c (c^T c - c^T B L^{\dagger} B^T c)^{-1} c^T B L^{\dagger}& - L^{\dagger} B^T c (c^T c - c^T B L^{\dagger} B^T c)^{-1} \\ -(c^T c - c^T B L^{\dagger} B^T c)^{-1} c^T B L^{\dagger} &   (c^T c - c^T B L^{\dagger} B^T c)^{-1}\end{array}\right].
$$
Now, in order to calculate $g^T (A^TA)^{\dagger}$, we can simply calculate $g^T L^{\dagger}$, $L^{\dagger} B^T c$ and $c^T B L^{\dagger} $. All these three vectors can be calculated in $\widetilde{O}(m)$ time using nearly-linear time Laplacian system solvers \cite{spielman2004nearly, koutis2010approaching, koutis2011nearly, lee2013efficient, kelner2013simple, cohen2014stretching, cohen2014preconditioning, kyng2016sparsified, kyng2016approximate}.


